Solving Dynamic Graph Problems with Multi-Attention Deep Reinforcement Learning

Graph problems such as traveling salesman problem, or finding minimal Steiner trees are widely studied and used in data engineering and computer science. Typically, in real-world applications, the features of the graph tend to change over time, thus, finding a solution to the problem becomes challenging. The dynamic version of many graph problems are the key for a plethora of real-world problems in transportation, telecommunication, and social networks. In recent years, using deep learning techniques to find heuristic solutions for NP-hard graph combinatorial problems has gained much interest as these learned heuristics can find near-optimal solutions efficiently. However, most of the existing methods for learning heuristics focus on static graph problems. The dynamic nature makes NP-hard graph problems much more challenging to learn, and the existing methods fail to find reasonable solutions. In this paper, we propose a novel architecture named Graph Temporal Attention with Reinforcement Learning (GTA-RL) to learn heuristic solutions for graph-based dynamic combinatorial optimization problems. The GTA-RL architecture consists of an encoder capable of embedding temporal features of a combinatorial problem instance and a decoder capable of dynamically focusing on the embedded features to find a solution to a given combinatorial problem instance. We then extend our architecture to learn heuristics for the real-time version of combinatorial optimization problems where all input features of a problem are not known a prior, but rather learned in real-time. Our experimental results against several state-of-the-art learning-based algorithms and optimal solvers demonstrate that our approach outperforms the state-of-the-art learning-based approaches in terms of effectiveness and optimal solvers in terms of efficiency on dynamic and real-time graph combinatorial optimization.

==> Arxiv-Udesh (1)/Tex/Tables.tex <==
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}

\pgfplotstableread[col sep = comma]{Tex/DataTSP.csv}\datatsp
\pgfplotstableread[col sep = comma]{Tex/DataVRP1.csv}\datavrp

\begin{figure*}[t]
\begin{subfigure}{0.30\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=5.8cm, height=4.8cm,     
grid=major, 
%xticklabels from table={\data}{Algorithm},
grid style={dashed,gray!30}, 
x tick label style={rotate=90},
ylabel=Tour Length,
ymin=2,
ylabel style={at={(0.1,0.5)}},
legend style={at={(0.5,-0.2)},anchor=north},
cycle list name=color list,
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={Gurobi, GTA-RL-bs(10), GTA-RL-bs(5), GTA-RL-greedy, GTA-RL-rt, NN, S2V-DQN-sorted, AM, RNN-RL, S2V-DQN-last}
]

\foreach \x in {0,..., 10}
    \addplot+[select coords between index={\x}{\x} , ybar, fill] table[x=index, y=TSP10, col sep=comma]{\datatsp};

\end{axis}
\end{tikzpicture}

\caption{Tour Length for TSP10}
\label{fig:tsp10}
\end{subfigure}\hspace{5mm}\begin{subfigure}{0.30\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=5.8cm, height=4.8cm,     
grid=major, 
%xticklabels from table={\data}{Algorithm},
grid style={dashed,gray!30}, 
x tick label style={rotate=90},
ylabel=Tour Length,
ymin=2,
ylabel style={at={(0.1,0.5)}},
legend style={at={(0.5,-0.2)},anchor=north},
cycle list name=color list,
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={Gurobi, GTA-RL-bs(10), GTA-RL-bs(5), GTA-RL-greedy, GTA-RL-rt, NN, S2V-DQN-sorted, AM, RNN-RL, S2V-DQN-last}
]

\foreach \x in {0,..., 10}
    \addplot+[select coords between index={\x}{\x} , ybar, fill] table[x=index, y=TSP20, col sep=comma]{\datatsp};

\end{axis}
\end{tikzpicture}

\caption{Tour Length for TSP20}
\label{fig:tsp20}
\end{subfigure}\hspace{5mm}\begin{subfigure}{0.30\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=5.8cm, height=4.8cm,     
grid=major, 
%xticklabels from table={\data}{Algorithm},
grid style={dashed,gray!30}, 
x tick label style={rotate=90},
ylabel=Tour Length,
ymin=6,
ylabel style={at={(0.1,0.5)}},
legend style={at={(0.5,-0.2)},anchor=north},
cycle list name=color list,
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={Gurobi, GTA-RL-bs(10), GTA-RL-bs(5), GTA-RL-greedy, GTA-RL-rt, NN, S2V-DQN-sorted, AM, RNN-RL, S2V-DQN-last}
]

\foreach \x in {0,..., 10}
    \addplot+[select coords between index={\x}{\x} , ybar, fill] table[x=index, y=TSP50, col sep=comma]{\datatsp};

\end{axis}
\end{tikzpicture}

\caption{Tour Length for TSP50}
\label{fig:tsp50}
\end{subfigure}
\caption{Tour length for dynamic TSP}

\end{figure*}

\begin{figure*}[t]
\begin{subfigure}{0.30\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=5.8cm, height=4.8cm,     
grid=major, 
%xticklabels from table={\data}{Algorithm},
grid style={dashed,gray!30}, 
x tick label style={rotate=90},
ylabel=Tour Length,
ymin=3,
ylabel style={at={(0.1,0.5)}},
legend style={at={(0.5,-0.2)},anchor=north},
cycle list name=color list,
xtick={1,2,3,4,5,6,7,8},
xticklabels={Gurobi, GTA-RL-bs(10), GTA-RL-bs(5), GTA-RL-greedy, GTA-RL-rt, AM-D, AM, RNN-RL}
]

\foreach \x in {0,..., 8}
    \addplot+[select coords between index={\x}{\x} , ybar, fill] table[x=index, y=VRP10, col sep=comma]{\datavrp};

\end{axis}
\end{tikzpicture}

\caption{Tour Length for VRP10}
\label{fig:vrp10}
\end{subfigure}\hspace{5mm}\begin{subfigure}{0.30\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=5.8cm, height=4.8cm,     
grid=major, 
%xticklabels from table={\data}{Algorithm},
grid style={dashed,gray!30}, 
x tick label style={rotate=90},
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend style={at={(0.5,-0.2)},anchor=north},
cycle list name=color list,
xtick={0,1,2,3,4,5,6,7,8},
ymin=6.5,
xticklabels={wild, Gurobi, GTA-RL-bs(10), GTA-RL-bs(5), GTA-RL-greedy, GTA-RL-rt, AM-D, AM, RNN-RL}
]

\foreach \x in {0,..., 7}
    \addplot+[select coords between index={\x}{\x} , ybar, fill] table[x=index, y=VRP20, col sep=comma]{\datavrp};

\end{axis}
\end{tikzpicture}

\caption{Tour Length for VRP20}
\label{fig:vrp20}
\end{subfigure}\hspace{5mm}\begin{subfigure}{0.30\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=5.8cm, height=4.8cm,     
grid=major, 
%xticklabels from table={\data}{Algorithm},
grid style={dashed,gray!30}, 
x tick label style={rotate=90},
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend style={at={(0.5,-0.2)},anchor=north},
cycle list name=color list,
%axis y discontinuity=crunch,
ymin=12,
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={wild, Gurobi, GTA-RL-bs(10), GTA-RL-bs(5), GTA-RL-greedy, GTA-RL-rt, AM-D, AM, RNN-RL}
]

\foreach \x in {0,..., 8}
    \addplot+[select coords between index={\x}{\x} , ybar, fill] table[x=index, y=VRP50, col sep=comma]{\datavrp};

\end{axis}
\end{tikzpicture}

\caption{Tour Length for VRP50}
\label{fig:vrp50}
\end{subfigure}
\caption{Tour length for dynamic VRP}
\vspace{-4mm}
\end{figure*}

==> Arxiv-Udesh (1)/Tex/critic.tex <==
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_9-tag-val_avg_reward.csv}\dataNine
\pgfplotstableread[col sep = comma]{Tex/run-run_28-tag-val_avg_reward.csv}\dataCritic
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_10-tag-val_avg_reward.csv}\dataTen
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_11-tag-val_avg_reward.csv}\dataElv
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_12-tag-val_avg_reward.csv}\dataTwe
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_14-tag-val_avg_reward.csv}\dataFteen

\begin{figure}[t]
\begin{tikzpicture}
 \begin{axis}[
width=9cm, height=4.8cm,     
%grid=major, 
%grid style={dashed,gray!30}, 
x tick label style={rotate=90},
xlabel=Epoch Number,
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend columns=3,
legend style={at={(0.5,0.7)},anchor=north, , font=\scriptsize, legend image post style={xscale=0.5}},
cycle list name=color list]


\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataNine};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataCritic};

\legend{GTA-RL-greedy (rollout), GTA-RL-Critic}
\centering
\end{axis}
\end{tikzpicture}
\caption{Tour length for validation data set for rollout and critic baselines}
\label{fig:val}
\vspace{-2mm}
\end{figure}

==> Arxiv-Udesh (1)/Tex/train.tex <==
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_9-tag-avg_cost.csv}\dataNine
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_10-tag-avg_cost.csv}\dataTen
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_11-tag-avg_cost.csv}\dataElv
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_12-tag-avg_cost.csv}\dataTwe
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_14-tag-avg_cost.csv}\dataFteen

\begin{figure}[t]
\begin{tikzpicture}
 \begin{axis}[
width=9cm, height=4.8cm,     
%grid=major, 
%grid style={dashed,gray!30}, 
x tick label style={rotate=90},
xlabel=Training Step,
ymax=8,
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend columns=3,
legend style={at={(0.54,0.98)},anchor=north, , font=\scriptsize, legend image post style={xscale=0.5}},
cycle list name=color list]


\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataNine};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataTen};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataElv};
\addplot+[green] table[x=Step, y, y=Value, col sep=comma]{\dataTwe};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataFteen};

\legend{GTA-RL-greedy, GTA-RL-sum, GTA-RL-(0), AM, GTA-RL-rt}
\centering
\end{axis}
\end{tikzpicture}
\caption{Tour length for training data set during the training}
%\vspace{-2mm}
\label{fig:trn}
\end{figure}

==> Arxiv-Udesh (1)/Tex/validation.tex <==
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_9-tag-val_avg_reward.csv}\dataNine
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_10-tag-val_avg_reward.csv}\dataTen
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_11-tag-val_avg_reward.csv}\dataElv
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_12-tag-val_avg_reward.csv}\dataTwe
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_14-tag-val_avg_reward.csv}\dataFteen

\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_9-tag-avg_cost.csv}\dataNineTrain
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_10-tag-avg_cost.csv}\dataTenTrain
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_11-tag-avg_cost.csv}\dataElvTrain
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_12-tag-avg_cost.csv}\dataTweTrain
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_14-tag-avg_cost.csv}\dataFteenTrain

\begin{figure}[t]
\begin{subfigure}{0.5\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=8.5cm, height=4.8cm,     
%grid=major, 
%grid style={dashed,gray!30}, 
x tick label style={rotate=90},
xlabel=Epoch Number,
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend columns=3,
legend style={at={(0.5,0.7)},anchor=north, , font=\scriptsize, legend image post style={xscale=0.5}},
cycle list name=color list]


\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataNine};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataTen};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataElv};
\addplot+[green] table[x=Step, y, y=Value, col sep=comma]{\dataTwe};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataFteen};

\legend{GTA-RL-greedy, GTA-RL-sum, GTA-RL-(0), AM, GTA-RL-rt}
\centering
\end{axis}
\end{tikzpicture}
\caption{Tour length for validation data set during the training}
\label{fig:val}
\vspace{-2mm}
\end{subfigure}\begin{subfigure}{0.5\columnwidth}
\begin{tikzpicture}
 \begin{axis}[
width=8.5cm, height=4.8cm,     
%grid=major, 
%grid style={dashed,gray!30}, 
x tick label style={rotate=90},
xlabel=Training Step,
ymax=8,
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend columns=3,
legend style={at={(0.54,0.98)},anchor=north, , font=\scriptsize, legend image post style={xscale=0.5}},
cycle list name=color list]


\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataNineTrain};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataTenTrain};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataElvTrain};
\addplot+[green] table[x=Step, y, y=Value, col sep=comma]{\dataTweTrain};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataFteenTrain};

\legend{GTA-RL-greedy, GTA-RL-sum, GTA-RL-(0), AM, GTA-RL-rt}
\centering
\end{axis}
\end{tikzpicture}
\caption{Tour length for training data set during the training}
%\vspace{-2mm}
\label{fig:trn}
\end{subfigure}
\end{figure}

==> Arxiv-Udesh (1)/Tex/visualize.tex <==
\begin{figure*}
\centering
\begin{subfigure}[t]{.35\textwidth}
\centering
    \includegraphics[width=5cm, height=3.6cm]{Figures/Picture1.pdf}
    \caption{AM with a tour length of 3.85}
    \label{fig:vis_a}
\end{subfigure}\begin{subfigure}[t]{.33\textwidth}
\centering
    \includegraphics[width=5cm, height=3.6cm]{Figures/Picture2.pdf}
        \caption{GTA-RL-greedy with a tour length of 3.15}
            \label{fig:vis_b}
\end{subfigure}\begin{subfigure}[t]{.33\textwidth}
\centering
    \includegraphics[width=5cm, height=3.6cm]{Figures/Picture3.pdf}
        \caption{Gurobi solution with a tour length 2.96}
            \label{fig:vis_c}
\end{subfigure}
\caption{Figure shows the order of selected nodes by AM, GTA-RL-greedy and Gurobi optimal solver. For easy visualization we use dynamic TSP10 where only 10 cities are present. The dots with the same color indicates the same city locations at different time steps. The black arrows shows the tour decision taken by each algorithm.}
\label{fig:visualize}
\end{figure*}

==> Tex/critic.tex <==
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_9-tag-val_avg_reward.csv}\dataNine
\pgfplotstableread[col sep = comma]{Tex/run-run_28-tag-val_avg_reward.csv}\dataCritic
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_10-tag-val_avg_reward.csv}\dataTen
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_11-tag-val_avg_reward.csv}\dataElv
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_12-tag-val_avg_reward.csv}\dataTwe
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_14-tag-val_avg_reward.csv}\dataFteen

\begin{figure}[t]
\begin{tikzpicture}
 \begin{axis}[
width=9cm, height=4.8cm,     
%grid=major, 
%grid style={dashed,gray!30}, 
x tick label style={rotate=90},
xlabel=Epoch Number,
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend columns=3,
legend style={at={(0.5,0.7)},anchor=north, , font=\scriptsize, legend image post style={xscale=0.5}},
cycle list name=color list]


\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataNine};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataCritic};

\legend{GTA-RL-greedy (rollout), GTA-RL-Critic}
\centering
\end{axis}
\end{tikzpicture}
\caption{Tour length for validation data set for rollout and critic baselines}
\label{fig:val}
\vspace{-2mm}
\end{figure}

==> Tex/train.tex <==
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_9-tag-avg_cost.csv}\dataNine
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_10-tag-avg_cost.csv}\dataTen
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_11-tag-avg_cost.csv}\dataElv
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_12-tag-avg_cost.csv}\dataTwe
\pgfplotstableread[col sep = comma]{Tex/run-icde_dynamic_tsp_20_run_14-tag-avg_cost.csv}\dataFteen

\begin{figure}[t]
\begin{tikzpicture}
 \begin{axis}[
width=9cm, height=4.8cm,     
%grid=major, 
%grid style={dashed,gray!30}, 
x tick label style={rotate=90},
xlabel=Training Step,
ymax=8,
ylabel=Tour Length,
ylabel style={at={(0.1,0.5)}},
legend columns=3,
legend style={at={(0.54,0.98)},anchor=north, , font=\scriptsize, legend image post style={xscale=0.5}},
cycle list name=color list]


\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataNine};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataTen};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataElv};
\addplot+[green] table[x=Step, y, y=Value, col sep=comma]{\dataTwe};
\addplot+[] table[x=Step, y, y=Value, col sep=comma]{\dataFteen};

\legend{GTA-RL-greedy, GTA-RL-sum, GTA-RL-(0), AM, GTA-RL-rt}
\centering
\end{axis}
\end{tikzpicture}
\caption{Tour length for training data set during the training}
%\vspace{-2mm}
\label{fig:trn}
\end{figure}
